Pairwise distortion distribution for compression and quantization

Choosing the latent dimension is a critical challenge in data compression, where conventional hyperparameter optimization is costly and ad hoc. Intrinsic dimension provides a good alternative, which connects information-theoretic notions such as Renyi information dimension (RID) to rate-distortion dimension and random codebook compression. In this work, we introduce the pairwise distortion distribution (PDD) and its asymptotic limit, pairwise dimension (PD), which generalize the correlation integral to general distortion measures. We show that PD bounds RID, and PDD provides a lower bound for random codebook quantization performance, which can guide a practical use for compression, quantization, and dimensionality reduction applications.

==> saved_pieces.tex <==
\begin{align}
    P\left[\Vert x-c\Vert_{2}^{2}
    
    \leq r\right] &= \int_{Y:\Vert Y \Vert\leq\sqrt{r}}\; p_{Y}\;(y)dy\\
    %&\stackrel{(a)}{\leq} p_y(0)\cdot \mbox{Vol}(B_{\sqrt{r}}(0))\\
    &\stackrel{(a)}{\leq} p_Y(0)\cdot \frac{\pi^{N/2}}{\Gamma(N/2+1)}r^{N/2}.
\end{align} where (a) is due to autocorrelation properties that the density achieves its maximum at the center with the assumption that $\mathcal{D}$ is a unimodal distribution centered at 0. %$\mbox{Vol}(B_{\sqrt{r}}(0))$ indicates the $N$-dimensional volume of a ball of radius $\sqrt{r}$. 
This yields $\beta=p_Y(0)\cdot \frac{\pi^{N/2}}{\Gamma(N/2+1)}$ and $d=N$ in \eqref{eq:cdf_approx}. 


\cn{Replace starting here}
When $r \rightarrow 0$, the pairwise dimension  $d_P(\mathcal{D},\rho)$ is characterized by $d$ by distributions whose $\pdd{\mathcal{D},\rho}{r}$ admits the form 
\begin{align}\label{eq:cdf_approx}
    \pdd{\mathcal{D},\rho}{r} \approx \beta r^{d/2}.
\end{align} When the CDF of the PDD takes this form, Proposition~\ref{prop:pdd_rcq} can be further characterized in terms of PD when a distortion measure $\rho(x,y)=\Vert x-y \Vert_2^2$.

\begin{proposition}Let $X \sim \mathcal{D}$ on $\mathbb{R}^{N}$ with pdf $p(X)$. Suppose that $\pdd{\mathcal{D},\rho}{r} \leq \min\{\beta r^{d/2},1\}$. We further characterize the bound in Proposition~\ref{prop:pdd_rcq} as
\begin{align}
        \mu 
    &\geq \frac{2}{\pi N} \left(\frac{\Gamma(N/2+1)}{p_Y(0)}\right)^{2/N} B(L+1,2/N),\label{eq:lb}
\end{align} where $\Gamma(\alpha)$ indicates the Gamma function and 
$B(z_1,z_2)$ is the beta function. $p_{Y}(y)$ is the pdf of the difference of two samples $X_1, X_2 \sim \mathcal{D}$ with $p(X)$,   $Y=X_1 - X_2$, $p_Y(y) = \int_{\mathbb{R}^{N}} \;p(X)p(X-Y)dx.$
\end{proposition}
\noindent\emph{Proof.} 
%Suppose that $x$ is drawn from $\mathcal{D}$ on $\mathbb{R}^{N}$ with the pdf $p(x)$. The distribution of the difference $y=x_{1}-x_2$ of two independent samples from $\mathcal{D}$ has the pdf $p_y(y) = \int_{\mathbb{R}^{N}} \;p(x)p(x-y)dx.$
\begin{align}
    \mu &\geq \int_0^\infty \left( 1-\pdd{\mathcal{D},\rho}{r}\right)^{L}\; dr\\
    &\geq \int_0^{\beta^{-2/d}} \left( 1-\beta r^{d/2}\right)^{L}\; dr \\
    &\geq \frac{2}{d}\beta^{-2/d}\int_{0}^{1}(1-\tau)^{L}\tau^{2/d-1} d\tau\\
    &\geq \frac{2}{d}\beta^{-2/d} \;B(L+1,2/d), \label{eq:lb_beta}
    %&\stackrel{(a)}{\geq} \frac{2}{d}\beta^{-2/d} \;\Gamma(2/d)(L+1)^{-2/d}, 
\end{align} where $B(z_1,z_2)$ is the beta function. 
\cn{cut to here}

For a distortion measure $\rho(x,y)=\Vert x-y \Vert_2^2$, we have
\begin{align}
    P\left[\Vert x-c\Vert_{2}^{2}\leq r\right] &= \int_{Y:\Vert Y \Vert\leq\sqrt{r}}\; p_{Y}\;(y)dy\\
    %&\stackrel{(a)}{\leq} p_y(0)\cdot \mbox{Vol}(B_{\sqrt{r}}(0))\\
    &\stackrel{(a)}{\leq} p_Y(0)\cdot \frac{\pi^{N/2}}{\Gamma(N/2+1)}r^{N/2}.
\end{align} where (a) is due to autocorrelation properties that the density achieves its maximum at the center with the assumption that $\mathcal{D}$ is a unimodal distribution centered at 0. %$\mbox{Vol}(B_{\sqrt{r}}(0))$ indicates the $N$-dimensional volume of a ball of radius $\sqrt{r}$. 
This yields $\beta=p_Y(0)\cdot \frac{\pi^{N/2}}{\Gamma(N/2+1)}$ and $d=N$ in \eqref{eq:cdf_approx}. 

